Robust Reinforcement Learning using Least Squares Policy Iteration with Provable Performance Guarantees

This paper addresses the problem of model-free reinforcement learning for Robust Markov Decision Process (RMDP) with large state spaces. The goal of the RMDP framework is to find a policy that is robust against the parameter uncertainties due to the mismatch between the simulator model and real-world settings. We first propose the Robust Least Squares Policy Evaluation algorithm, which is a multi-step online model-free learning algorithm for policy evaluation. We prove the convergence of this algorithm using stochastic approximation techniques. We then propose Robust Least Squares Policy Iteration (RLSPI) algorithm for learning the optimal robust policy. We also give a general weighted Euclidean norm bound on the error (closeness to optimality) of the resulting policy. Finally, we demonstrate the performance of our RLSPI algorithm on some standard benchmark problems.

==> ICML 2021 Submission/01-Introduction.tex <==
\section{Introduction}

Model-free Reinforcement Learning (RL) algorithms typically learn a policy by training on a simulator. In  the RL literature, it is nominally assumed that the testing environment is identical to the training environment (simulator model). However, in reality, the parameters of the simulator model can be different from the real-world setting. This can be due to the approximation errors incurred while modeling, due to the changes in the real-world parameters over time, and can even be due to possible adversarial  disturbances in the real-world.  For example, in many robotics applications,  the standard simulator parameter settings  (mass, friction,  wind conditions, sensor noise, action delays) can be different from that of the actual robot in the real-world.  This mismatch between   the training and testing environment  parameters  can significantly degrade the real-world performance of the model-free learning algorithms trained on a simulator model.


%The RMDP formulation considers a set of model parameters (uncertainty set) under the assumption that the actual parameters lie in this  uncertainty set, and the  algorithm computes a robust policy that performs  best under the worst model. 


The RMDP framework \citep{iyengar2005robust, nilim2005robust}  addresses the \textit{planning} problem of computing the optimal policy  that is robust against parameter uncertainties that cause the mismatch between the training and testing environment  parameters. The RMDP problem has been analyzed extensively in the tabular case \citep{iyengar2005robust, nilim2005robust, wiesemann2013robust, xu2010distributionally, yu2015distributionally} and  under the linear function approximation \citep{tamar2014scaling}. Algorithms for learning the optimal robust policy  with provable guarantees  have  been proposed, both in the model-free  \citep{roy2017reinforcement} and model-based \citep{lim2013reinforcement}   reinforcement learning settings.   However, the theoretical guarantees from these works are limited to  the tabular RMDP settings.  Learning policies for problems  with  large state spaces is computationally  challenging. RL algorithms typically overcome this issue by using function approximation architectures, such as  linear basis functions \citep{lagoudakis2003least}, reproducing kernel Hilbert spaces (RKHS) \citep{yang2020reinforcement} and deep neural networks \citep{lillicrapHPHETS15}. Recently, robust reinforcement learning problem has been addressed  using deep RL methods  \citep{pinto2017robust, Mankowitz2020Robust, zhang2020robust, derman2018soft, vinitsky2020robust}. However, these works are  empirical in nature and do not provide any theoretical guarantees for the learned policies. The problem of learning optimal robust policies with provable performance guarantees for RMDPs with  large state spaces  has not been well studied in the literature.  








% \citep{roy2017reinforcement}    studied the simulation based  policy evaluation using function approximation, but did not address the problem of learning the optimal robust policy.







% \redtext{It is widely known that, complexity of methods such as dynamic programming and other tabular RL methods scales linearly with the number of states, often referred as ``curse of dimensionality”, hence becoming intractable for solving practical problems. Many RL methods are able to alleviate this curse by data sampling (giving raise to high confidence results) and by function approximation architectures (expanding the original state space into a higher dimensional state space). One of such RL methods is the approximate dynamic programming (ADP) \citep{bertsekas2011approximate} which use linear function approximation architectures in their models. Of course, use of non-linear function approximation architectures further expands the original state space into a vastly higher dimensional state space, nevertheless, from the experience of picking good features ADP has been used successfully in large-scale problems \citep{tamar2014scaling,roy2017reinforcement,kaufman2013robust}. Witnessing such empirical success of ADP in achieving robust solutions to practical problems,} 


 
% We focus on the approach of least squares based online model-free reinforcement learning with linear function approximation for learning a policy that is robust against the parameter uncertainties.  
 
In this paper, we address the problem of learning a  policy that is provably robust against the parameter uncertainties for RMDPs with  large state spaces. In particular, we propose an online model-free reinforcement learning algorithm with linear function approximation for learning the optimal robust policy, and provide theoretical guarantees on the performance of the learned policy.   Our choice of  linear function approximation is motivated by its analytical tractability while providing the scaling to large  state  spaces. Indeed, linear function approximation based approaches have been successful in providing algorithms with provable guarantees for many challenging problems in RL, including online model-free exploration \citep{jin2020provably,yang2020reinforcement}, imitation learning \citep{abbeel2004apprenticeship,arora2020provable}, meta reinforcement learning \citep{wang2020global,kong2020meta}, and offline reinforcement learning \citep{wang2021what,duan2020minimax}. Robust RL is much more challenging than the standard  (non-robust) RL problems due to the inherent  nonlinearity associated with the robust dynamic programming.  We overcome this issue by a cleverly designed approximate dynamic programming approach. We then propose a model-free robust policy iteration using this approach  with provable guarantees.  Our algorithmic and technical contributions are as follows:

(i) Robust Least Squares Policy Evaluation (RLSPE($\lambda$)) algorithm: A learning-based policy iteration algorithm  needs to learn  the value of a policy for performing (greedy) policy improvement. For this, we first propose RLSPE($\lambda$) algorithm, a multi-step, online, model-free policy evaluation algorithm with linear function approximation. This can be thought as the  robust version of classical least squares based RL algorithms for policy evaluation, like LSTD($\lambda$) and LSPE($\lambda$). We  prove the convergence of this algorithm using stochastic approximation techniques, and also  characterize its approximation error due to the linear architecture. 
% To the best of our knowledge, this is the first work that presents least squares based online model-free policy evaluation algorithms for robust reinforcement learning problems with provable guarantees.  

(ii) Robust Least Squares Policy Iteration (RLSPI) algorithm: We  propose the RLSPI  algorithm for learning the optimal robust policy. We also give a general $L_{2}$-norm bound on the error (closeness to optimality) of the resulting policy at any iterate of the algorithm. To the best of our knowledge, this is the first work that presents a learning based policy iteration algorithm for robust reinforcement learning with such provable guarantees.  

(iii)  Finally, we demonstrate the performance of the RLSPI algorithm on various  standard RL test environments.

% from OpenAI Gym \citep{brockman2016openai}, like, CartPole, MountainCar, Acrobot environments in the MushroomRL library \citep{deramo2020mushroomrl}.






%Similar to the framework in \citep{roy2017reinforcement}, we assume that a nominal simulator is available for model-free learning and the parameter uncertainty set is characterized with respect to the nominal but unknown simulator model parameters. 

\subsection{Related Work}
RMDP formulation to address the parameter uncertainty problem was first proposed by \citep{iyengar2005robust} and \citep{nilim2005robust}. \citep{iyengar2005robust} showed that the optimal robust value function and policy can be computed using the robust counterparts of the standard value iteration and policy iteration.  To tackle the parameter uncertainty problem, other works considered distributionally robust setting \citep{xu2010distributionally}, modified policy iteration \citep{kaufman2013robust}, and {more general uncertainty set} \citep{wiesemann2013robust}. We note that the focus of these works were mainly on the planning problem in the tabular setting.  Linear function approximation method to solve large  RMDPs was proposed in \citep{tamar2014scaling}. Though this work suggests a sampling based approach, a general model-free learning algorithm and analysis was not included. \citep{roy2017reinforcement} proposed the robust versions of the classical model-free  reinforcement learning algorithms such as Q-learning, SARSA, and TD-learning in the tabular setting. They also proposed function approximation based algorithms for  the policy evaluation. However,  this work does not have a policy iteration algorithm with provable guarantees for learning the optimal robust policy.   \citep{derman2018soft}  introduced soft-robust actor-critic algorithms using neural networks, but does not provide any global convergence  guarantees for the learned policy. \citep{tessler2019action} proposed a min-max game framework to address the robust learning problem focusing on the tabular setting. \citep{lim2019kernel}  proposed a kernel-based RL algorithm for finding the robust value function in a batch learning setting.  \citep{Mankowitz2020Robust} employed an entropy-regularized policy optimization algorithm for continuous control using neural network, but does not provide any provable guarantees for the learned policy.  



% framework and policy iteration approach based solution, \redtext{giving guarantees only for the tabular MDPs case.}

% \redtext{for which they only establish convergence to a local optimum of their soft-robust objective function.}  

% \redtext{for which they provided guarantees only for the robust policy evaluation and not for the policy improvement step.} \citep{lim2019kernel}  proposed a kernel-based RL algorithm for finding the robust value function \redtext{by constructing a model using the state-action trajectories generated by policies in the policy update step.} \citep{derman2018soft}  introduced soft-robust actor-critic algorithms \redtext{for which they only establish convergence to a local optimum of their soft-robust objective function.}    \citep{tessler2019action} proposed  a probabilistic action robust game-theoretic framework and policy iteration approach based solution, \redtext{giving guarantees only for the tabular MDPs case.} \citep{Mankowitz2020Robust} employed an entropy-regularized policy optimization algorithm for continuous control, \redtext{providing guarantees only for the policy evaluation steps}. 


Our work differs from the above in two significant ways. Firstly, we  develop a new multi-step model-free reinforcement learning algorithm, RLSPE($\lambda$), for policy evaluation.  Extending the classical least squares based policy evaluation algorithms, like LSPE($\lambda$) and LSTD($\lambda$) \citep{BerBook12}, to the robust case is very challenging due to the nonlinearity of the robust TD($\lambda$) operator. We overcome this issue by a cleverly defined approximate  robust TD($\lambda$) operator that is amenable to online learning using least squares approaches. Also, as pointed out in \citep{bertsekas2011approximate}, convergence analysis of least squares style algorithms for RL is different from that of the standard temporal difference (TD) algorithm. Secondly, we develop a new robust policy iteration algorithm with provable guarantees on the performance of the policy at any iterate. In particular, we give a general weighted Euclidean norm bound on the error of the resulting policy. While similar results are available for the non-robust settings, this is the first work to provide such a characterization in the challenging setting of robust reinforcement learning. 










==> ICML 2021 Submission/02-Formulation.tex <==

\section{Background and Problem Formulation}
\label{sec:formulation}

A Markov Decision Process is a tuple $M = (\Ss, \Aa, r, P, \alpha)$ where $\Ss$ is the  state space, $\Aa$ is the  action space,  $r: \Ss\times \Aa\rightarrow \R$ is the reward function, and $\alpha \in (0, 1)$ is the discount factor. The transition probability matrix $P_{s,a}(s')$ represents the probability of transitioning to state $s'$ when  action $a$ is taken at state $s$. We consider a finite MDP setting where the cardinality of state and action spaces are finite (but very large).    A  policy $\pi$ maps each state to an action. The value of a policy $\pi$ evaluated at state $s$ is given by
\begin{align*}
V_{\pi, P}(s) = \E_{\pi, P}[\sum^{\infty}_{t=0} \alpha^{t} r(s_{t}, a_{t}) ~|~ s_{0} = s], \end{align*}where $a_{t} \sim \pi(s_{t})$ and $s_{t+1} \sim P_{s_t,a_t}(\cdot)$. The optimal  value function and the  optimal policy of an MDP with the transition probability $P$ is defined as $V^{*}_{P} = \max_{\pi} V_{\pi, P}$ and $\pi^{*}_{P} = \argmax_{\pi} V_{\pi, P}$. 



% Moreover, the rectangularity condition ensures that the worst-case transition happens independently for all state-action pairs.
The RMDP formulation considers a set of model parameters (uncertainty set) under the assumption that the actual parameters lie in this  uncertainty set, and the  algorithm computes a robust policy that performs  best under the worst model.  More precisely, instead of a fixed  transition probability matrix $P$, we consider a set of transition probability matrices $\mathcal{P}$.  We assume that the set $\mathcal{P}$ satisfies the standard \textit{rectangularity condition} \citep{iyengar2005robust}. The objective is to find a policy that maximizes the worst-case performance.  Formally, the \textit{robust value function} $V_{\pi}$ corresponding to a policy $\pi$ and the \textit{optimal robust value function} $V^{*}$ are defined as
\citep{iyengar2005robust,nilim2005robust}
\begin{align}
\label{eq:Vpi-Vstart-1}
V_{\pi} = \inf_{P \in \mathcal{P}} ~V_{\pi, P},~~ V^{*} = \sup_{\pi} \inf_{P \in \mathcal{P}} ~V_{\pi, P} . 
\end{align} 
The \textit{optimal robust policy} $\pi^{*}$ is such that the robust value function corresponding to it matches the optimal robust value function, that is, $V_{\pi^*} =V^{*} $.

A generic characterization of the set  $\mathcal{P}$ makes the RMDPs problems intractable to solve by model-free methods. In the standard model-free methods, the algorithm has access to a simulator that can simulate the next state given the current state and current action, according to a fixed transition probability matrix (that is unknown to the algorithm). However, generating samples according to each and every transition probability matrix from the set $\mathcal{P}$ is clearly infeasible. To overcome this difficulty, we use the characterization of the uncertainty set used in \citep{roy2017reinforcement}. 
\begin{assumption}[Uncertainty Set]
Each $P \in \mathcal{P}$ can be represented as $P_{s,a}(\cdot) = P^{o}_{s,a}(\cdot) + U_{s,a}(\cdot)$ for some $U_{s,a} \in \mathcal{U}_{s,a}$, where $P^{o}_{s,a}(\cdot)$ is the unknown transition probability matrix corresponding to the nominal (simulator) model and $\mathcal{U}_{s,a}$ is a confidence region around it. 
\end{assumption}
Using the above characterization, we can write $\mathcal{P} = \{P^{o} + U : U \in \mathcal{U} \}$, where $\mathcal{U} = \cup_{s,a} \mathcal{U}_{s,a}$. So,  $\mathcal{U}$ is the set of all possible perturbations to the nominal model $P^{o}$. 


An example of the uncertainty set $\U$ can be the spherical uncertainty set with a radius parameter.  Define $\U_{s,a}:= \{ x~|~\|x\|_2 \leq r, \sum_{s\in\Ss} x_s = 0, -P^o_{s,a}(s') \leq x_{s'} \leq 1-P^o_{s,a}(s'), \forall s' \in \Ss \},$ for all $(s,a)\in(\Ss,\Aa)$, for some  $r>0$. Notice that, this uncertainty set uses the knowledge of the nominal model $P^o$ in its construction. In practice, we do not know $P^o$. So,  in Section \ref{sec:rlspe-1}, we introduce an approximate uncertainty set without using this information. 

We consider \textit{robust Bellman operator for policy evaluation}, defined as \citep{iyengar2005robust}
\begin{align}
\label{eq:Tpi-basic}
\hspace*{-0.2cm} T_{\pi} (V) (s) =  r(s,\pi(s)) + \alpha \inf_{P \in \mathcal{P}}   \sum_{s'} P_{s,\pi(s)}(s') V(s'),\hspace*{-0.2cm}
\end{align} a popular approach to solve \eqref{eq:Vpi-Vstart-1}. Using our characterization of the uncertainty set, we can rewrite \eqref{eq:Tpi-basic} as
\begin{align}
\label{eq:Tpi-1}
T_{\pi} (V) (s) &=  r(s,\pi(s)) + \alpha  \sum_{s'} P^{o}_{s,\pi(s)}(s') V(s') \nonumber \\&\hspace{0.5cm}+ \alpha \inf_{U \in \mathcal{U}_{s,\pi(s)}}   \sum_{s'} U_{s,\pi(s)}(s') V(s').
\end{align}
For any set  $\mathcal{B}$ and a vector $v$, define $
\sigma_{\mathcal{B}} (v) = \inf \{ u^{\top}v : u \in \mathcal{B} \}.$ We denote $|\Ss|$ as the cardinality of the set $\Ss$. Let ${\sigma}_{\mathcal{U}_\pi} (v)$ and  $r_{\pi}$ be the $|\mathcal{S}|$ dimensional column vectors defined as $ (\sigma_{\mathcal{U}_{s,\pi(s)}}(v) : s \in \mathcal{S})^{\top}$ and   $(r(s,\pi(s)): s \in \mathcal{S})^\top$, respectively. Let  $P^{o}_{\pi}$ be the stochastic matrix corresponding to the policy $\pi$ where for any $s,s'\in\Ss,$ $P^{o}_{\pi}(s,s') = P^{o}_{s,\pi(s)}(s')$. Then, \eqref{eq:Tpi-1} can be written in the matrix form as
\begin{align}
\label{eq:Tpi-matrix-1}
T_{\pi} (V)  =  r_{\pi} + \alpha  P^{o}_{\pi} V + \alpha \sigma_{U_{\pi}} (V).
\end{align}
It is known  \citep{iyengar2005robust} that $T_{\pi}$ is a contraction in sup norm and the robust value function $V_{\pi}$ is the unique fixed point of $T_{\pi}$. The \textit{robust Bellman operator} $T $ can also be defined in the same way as in the non-robust setting,
\begin{align}
\label{eq:T}
T (V)  =  \max_{\pi}T_{\pi} (V).
\end{align}
It is also known   \citep{iyengar2005robust} that $T$ is a contraction in sup norm, and the optimal robust value function $V^{*}$   is its unique fixed point. 

The goal of the robust RL is to learn the optimal robust policy $\pi^{*}$ without knowing the nominal model $P^{o}$ or the uncertainty set $\mathcal{P}$. 


%In particular, we first propose  RLSPE($\lambda$) algorithm for policy evaluation in the next section. Using this RLSPE($\lambda$) algorithm, we propose RLSPI algorithm for learning the optimal policy in section \ref{kk}. 


% We now give a specific example for the confidence region $\U_{s,a}$. Let $\{B_s^a \}_{s,a}$ be a sequence of $n\times n$ invertible matrices. Then we can define an ellipsoid confidence region as \[ \U_s^a := \left\{ x~\Bigg|~ x^\top B_s^a x \leq 1, \sum_{s\in\Ss} x_s = 0, -P^{o}_{s,a}(s') \leq x_{s'} \leq 1-P^{o}_{s,a}(s'), \forall s' \in \Ss \right\}. \] Since the probability vector $P^{o}_{s,a}$ is unknown for all $(s,a)$, we use a proxy confidence region $\widehat{\U}_{s,a}$ instead of $\U_{s,a} $ defined as \[  \widehat{\U}_{s,a} := \left\{ x~\Bigg|~ x^\top B_s^a x \leq 1, \sum_{s\in\Ss} x_s = 0 \right\}. \] Supposing $\{B_s^a \}_{s,a}=A$ for a diagonal matrix $A$ with entries $r$ in the diagonal, then every uncertainty set $\Pp_{s,a}$ is an $\ell_2$ ball of radius $r$.

==> ICML 2021 Submission/03-LSPE.tex <==
\section{Robust Least Squares Policy Evaluation}
\label{sec:RPE}  
In this section, we develop the RLSPE($\lambda$) algorithm for learning the robust value function.
% $V_{\pi}$ for a given policy.

\subsection{Robust TD$(\lambda)$ Operator and the Challenges}  
\label{sec:RTB-Ber}
In RL,  a very useful approach for analyzing the multi-step learning algorithms  like TD($\lambda$), LSTD($\lambda$), and LSPE($\lambda$) is to define a multi-step Bellman operator called  TD($\lambda$) operator \citep{tsitsiklis1997analysis} \citep{BerBook12}.  Following the same approach, we can define  the robust TD($\lambda$) operator as well. For a given policy $\pi$, and a parameter $\lambda \in [0, 1),$ the robust TD($\lambda$) operator denoted by ${T}^{(\lambda)}_\pi : \mathbb{R}^{|\mathcal{S}|} \rightarrow \mathbb{R}^{|\mathcal{S}|}$ is defined as
\begin{align}
\label{eq:TLambda-Ber-1}
{T}^{(\lambda)}_\pi (V )= (1-\lambda) \sum_{m=0}^\infty \lambda^{m} T^{m+1}_{\pi}(V). 
\end{align} 
Note that for $\lambda = 0,$ we recover $T_{\pi}$. The following result is straightforward.
\begin{proposition}[informal]
\label{prop:informal-cont-fp-1}
${T}^{(\lambda)}_\pi$ is a contraction in  sup norm  and  the robust value function $V_{\pi}$ is its unique fixed point, for any $\alpha \in (0, 1), \lambda \in [0, 1)$.
\end{proposition}


% We can show that \emph{${T}^{(\lambda)}_\pi$ is a contraction in the sup norm  and  the robust value function $V_{\pi}$ is its unique fixed point, for any $\alpha \in (0, 1), \lambda \in [0, 1)$}. The precise  statements of this result and proof is given in the supplementary material.   

% Using the contraction property, $V_{\pi}$ can be computed by iteratively applying   $T_{\pi}$ or ${T}^{(\lambda)}_\pi$.   

For RMDPs with very large state space, exact dynamic  programming methods which involve  the evaluation of \eqref{eq:Tpi-1} or \eqref{eq:TLambda-Ber-1} are intractable.  A standard approach to overcome this issue is to approximate the value function using some function approximation architecture. Here we focus on linear function approximation architectures \citep{BerBook12}. In linear function approximation architectures, the value function is represented as the weighted sum of features as, $\bar{V}(s) = \phi(s)^{\top} w, \forall s \in \mathcal{S},$ where $ \phi(s)  = (\phi_{1}(s), \phi_{2}(s), \ldots, \phi_{L}(s))^{\top}$ is an $L$ dimensional feature vector with $L < |\mathcal{S}|$, and  $w = (w_1,\cdots,w_{L})^\top$ is a weight vector. In the matrix form, this can be written as $\bar{V} = \Phi w $ where  $\Phi$ is an $|\mathcal{S}| \times L$  dimensional feature matrix whose $s^{\text{th}}$ row  is $\phi(s)^{\top} $. We assume linearly independent columns for $\Phi$, i.e., rank($\Phi$) = $L$. 

The standard approach to find an approximate (robust) value function is  to solve for  a $w_{\pi}$, with $\bar{V}_{\pi} =  \Phi
 w_{\pi}$, such that $\Phi w_{\pi} = \Pi T^{(\lambda)}_{\pi} \Phi w_{\pi}$, where $\Pi$ is a   projection  onto the subspace spanned by the columns of $\Phi$. The projection is with  respect to a $d$-weighted  Euclidean norm. This norm is defined as  $\| V \|^{2}_{d} =  V^{\top} D V$, where $D$ is a diagonal matrix with non-negative diagonal entries $(d(s), s \in \mathcal{S})$, for any  vector $V$. Under suitable assumptions, \citep{tamar2014scaling} showed that $\Pi T_{\pi}$ is a contraction in a  $d$-weighted  Euclidean norm. We also use a similar assumption stated below.
\begin{assumption}
\label{as:offpolicy}
(i) For any given policy $\pi$, there exists an exploration policy $\pi_{e} =  \pi_{\text{exp}}(\pi)$ and a $\beta \in (0,1)$ such that $\alpha P_{s,\pi(s)}(s') \leq \beta P^{o}_{s,\pi_{e}(s)}(s')$, for all transition probability matrices $P\in\Pp$ and for all states $s,s'\in\Ss$.  \\
(ii) There exists a steady state distribution $d_{\pi_{e}} = (d_{\pi_{e}}(s), s \in \mathcal{S})$ for the Markov chain with transition probability $P^{o}_{\pi_{e}}$ with $d_{\pi_{e}}(s) > 0, \forall s \in \mathcal{S}$.
\end{assumption}
In the following, we will simply use $d$ instead of $d_{\pi_{e}}$. 
% \redtext{Note that we call a policy an \emph{exploration policy} when the data sampling by an algorithm is carried out using it.} 


% \begin{assumption}
% \label{as:offpolicy}
% (i) Let $\hat{\pi}$ be a given exploration policy.	There exists $\beta \in (0,1)$ such that $\alpha P_{s,\pi(s)}(s') \leq \beta P^{o}_{s,\hat{\pi}(s)}(s')$, for all transition probability matrices $P\in\Pp$, for all states $s,s'\in\Ss$, and for all policies $\pi$.\\
% (ii) There exists a steady state distribution $d = (d_{s}, s \in \mathcal{S})$  induced by the exploration policy $\hat{\pi}$ on the MDP with transition probability matrix $P^{o}$ with $d_{s} > 0, \forall s \in \mathcal{S}$.
% \end{assumption}


Though the above assumption appears restrictive, it is necessary to show that  $\Pi T_{\pi}$  is a contraction in the $d$-weighted Euclidean norm, as proved in \citep{tamar2014scaling}. Also, a similar assumption is used in proving the convergence of off-policy reinforcement learning algorithm  \citep{bertsekas2009projected}. In the robust case, we can expect a similar condition because  we are learning a robust value function for a set of transition probability matrices instead of a single transition probability matrix. We can now show the following. 

\begin{proposition}[informal]
\label{prop:informal-cont-fp-2}
Under Assumption \ref{as:offpolicy}, $\Pi {T}^{(\lambda)}_\pi$ is a contraction mapping in the $d$-weighted Euclidean norm for any $\lambda \in [0, 1)$. 
\end{proposition}


% Let $d_{\pi_{e}}$ (denoted only as $d$ from here onwards) be the steady state distribution of the Markov chain $P^{o}_{\pi_{e}}$ where $\pi_{e} =\pi_{\text{exp}}(\pi)$. Using the above assumption, we can show that 
% $\Pi {T}^{(\lambda)}_\pi$ is a contraction mapping in the $d$-weighted Euclidean norm for any $\beta \in (0, 1), \lambda \in [0, 1)$. The precise  statement of this result and proof are given in the supplementary material. 


The linear approximation based robust value function $\bar{V}_{\pi} =\Phi w_{\pi}$ can be computed using the iteration, $\Phi w_{k+1} = \Pi T^{(\lambda)}_{\pi} \Phi w_{k}$. Since  $\Pi T^{(\lambda)}_{\pi}$ is a contraction, $w_{k}$ will converge to $w^{*}$.  A closed form solution for $w_{k+1}$ given $w_{k}$ can be found by {\bf least squares approach} as $
w_{k+1} = \arg \min_{w} \|\Phi w - \Pi T^{(\lambda)}_{\pi} \Phi w_{k}\|^{2}_{d}$. It can be shown that (details are given in the supplementary material), we can get a closed form solution for $w_{k+1}$  as \begin{align}
\label{eq:rpvi-11} 
w_{k+1} = w_{k} + (\Phi^{\top} D \Phi)^{-1} \Phi^{\top} D (T^{(\lambda)}_{\pi} \Phi w_{k}  - \Phi w_{k}). 
\end{align}This is similar to the  projected equation approach \citep{BerBook12} in the non-robust setting. Even in the non-robust setting,  iterations using the \eqref{eq:rpvi-11} is intractable for MDPs with large state space. Moreover, when the transition  matrix is unknown, it is not feasible to use \eqref{eq:rpvi-11} exactly  even for small RMDPs.  Simulation-based model-free learning algorithms are developed for addressing this problem in the  non-robust case.  In particular, LSPE($\lambda$) algorithm   \citep{nedic2003least, BerBook12}  is used to solve the iterations of the above form. 


However, compared to the non-robust setting, there are two significant challenges in learning the robust value function  by  using simulation-based model-free approaches.

%can be expressed as $\bar{T}^{(\lambda)}_{\pi}$ can be written as $\bar{T}^{(\lambda)}_{\pi} V = r^{(\lambda)}_{\pi} + \alpha P^{(\lambda)}_{\pi} V $ where $r^{(\lambda)}_{\pi} = \sum^{\infty}_{m=0} \alpha^{m} \lambda^{m} (P^{o}_{\pi})^{m} r_{\pi},  P^{(\lambda)}_{\pi} = (1 - \lambda) \sum^{\infty}_{m=0} \alpha^{m} \lambda^{m} (P^{o}_{\pi})^{m+1}$ \citep{Berbook}. Since it doesn't involve any nonlinear operation, it can be  estimated using simulation-based model-free approaches as shown in \citep{Berbook}
(i) Non-linearity of the robust TD($\lambda$) operator:  The non-robust $T_{\pi}$ operator and the TD($\lambda$)  operator do not involve any nonlinear operations. So, they can be estimated efficiently from simulation samples in  a model-free way.  However, the robust TD($\lambda$) operator when expanded will have the  following form (derivation is given in the supplementary material).
\begin{align}
\label{eq:TLambda-Ber-expanded}
T^{(\lambda)}_{\pi}(V) &= (1 - \lambda) \sum^{\infty}_{m=0} \lambda^{m} (\sum^{m}_{k=0} (\alpha P^{o}_{\pi})^{k} r_{\pi} + (\alpha P^{o}_{\pi})^{m+1} V \nonumber \\&\hspace{1cm}+ \alpha \sum^{m}_{k=0} (\alpha P^{o}_{\pi})^{k} \sigma_{\mathcal{U}_{\pi}} (T^{(m-k)}_\pi V)). 
\end{align}
The last term is very difficult to estimate using simulation-based model-free approaches due to the composition of operations $\sigma_{\U_{\pi}}$ and $T_\pi$. In addition, nonlinearity of the $T_{\pi}$ operator by itself adds to the complexity. 
%$\sum^{m}_{k=0} (\alpha P^{o}_{\pi})^{k} \sigma_{\mathcal{U}_{\pi}} (T^{(m-k)}_\pi V)$ 


(ii) Unknown uncertainty region $\mathcal{U}$: In our formulation, we assumed that the transition probability uncertainty  set $\mathcal{P}$ is given by $\mathcal{P} = P^{o} + \mathcal{U}$. So, for each $U \in \mathcal{U}$, $ P^{o} + U$ should be a valid transition probability matrix. However, in the model-free setting, we do not know the nominal transition probability $P^{o}$. So, it is not possible to know $ \mathcal{U}$ exactly a priori. One can only use an approximation  $	\widehat{\U}$ instead of $\mathcal{U}$. This can possibly affect the convergence of the learning algorithms. 



\subsection{Robust Least Squares Policy Evaluation (RLSPE($\lambda$)) Algorithm } 
\label{sec:rlspe-1}
We overcome  the challenges of learning the robust value function by defining an   approximate robust TD($\lambda$) operator, and by developing a robust least squares policy evaluation algorithm based on that. 

Let $\widehat{\mathcal{U}}$ be the approximate uncertainty set we use instead of the actual uncertainty set. An example of the approximate uncertainty set $\widehat{\mathcal{U}}$ can be the spherical uncertainty set defined \textit{without} using the knowledge of the model $P^{o}$ as   $\widehat{\U}_{s,a}:= \{ x~|~\|x\|_2 \leq r, \sum_{s\in\Ss} x_s = 0\}$ for all $(s,a)\in(\Ss,\Aa)$. Note that $P^{o} + U$ for $U \in \widehat{\mathcal{U}}$ need not be a valid transition probability matrix and this poses challenges both for the algorithm and analysis. 









For a given policy $\pi$ and a parameter $\lambda \in [0, 1),$ approximate robust TD($\lambda$) operator denoted by $\widetilde{T}^{(\lambda)}_\pi : \mathbb{R}^{|\mathcal{S}|} \rightarrow \mathbb{R}^{|\mathcal{S}|},$ is defined as
\begin{align}
\label{eq:TLambda-1}
\widetilde{T}^{(\lambda)}_\pi (V )&= (1-\lambda) \sum_{m=0}^\infty \lambda^{m} \left[\sum_{t=0}^{m} (\alpha P^{o}_\pi)^t {r}_\pi \right. \nonumber \\&\hspace{0.1cm} \left. + \alpha \sum_{t=0}^{m} (\alpha P^{o}_\pi)^t  ~ {\sigma}_{\widehat{\U}_\pi} (V) + (\alpha P^{o}_\pi)^{m+1} V \right].
\end{align}
Note that even with $\widehat{\U}_\pi = {\U}_\pi$,  \eqref{eq:TLambda-1} is different from \eqref{eq:TLambda-Ber-expanded}. We will  show that this clever approximation  helps to overcome the  challenges due to the nonliterary associated with \eqref{eq:TLambda-Ber-expanded}.

However, we emphasize that \eqref{eq:TLambda-1} is not an arbitrary definition. Note that, for $\widehat{\U}_\pi = {\U}_\pi$, with $\lambda = 0,$ we recover the operator $T_{\pi}$. Moreover, the robust value function $V_{\pi}$ is a fixed point of $\widetilde{T}^{(\lambda)}_\pi $ when  $\widehat{\U}_\pi = {\U}_\pi$ for any $\lambda \in [0, 1).$ We state this formally below. 


%\begin{remark}
%Robust TD($\lambda$) operator can be defined in other ways also. One approach is to naively use the standard  TD($\lambda$) operator definition  $(1-\lambda) \sum^{\infty}_{m=0} \lambda^{m} T^{m+1}_{\pi}$   as given in \citep{BerBook}.  However, in the robust case, the nonlinearity of the infimum operation inside $T_{\pi}$ will make it a complicated  form which is not amenable to a least squares style learning algorithm. We define the robust TD($\lambda$) operator as above because it satisfies all the necessary properties and it is amenable to least squares style learning approaches as we show in the following sections.  
%\end{remark}
%the standard  TD($\lambda$) operator definition \citep{TV97}  as 
%\[ \inf_{P_{\pi} \in \mathcal{P}_{\pi}} ((1-\lambda) \sum^{\infty}_{\lambda = 0} \lambda^{m} (\sum^{m}_{t=0} (\alpha P_{\pi})^{t} r_{\pi} + \sum^{m}_{t=0} (\alpha P_{\pi})^{t} V  +  (\alpha P_{\pi})^{m+1} V )). \]
%Another approach is to use In the non-robust case,  both definitions are equivalent.

% We first show that, even though the definition  \eqref{eq:TLambda-1} is different from \eqref{eq:TLambda-Ber-expanded}, the robust value function $V_{\pi}$ is a fixed point of $\widetilde{T}^{(\lambda)}_\pi $ when  $\widehat{\U}_\pi = {\U}_\pi$.
\begin{proposition}
\label{prop:fixedpoint-1}
Suppose $\widehat{\U}_\pi = {\U}_\pi$. Then, for any $\alpha \in(0, 1)$ and  $\lambda \in [0, 1),$ the robust value function $V_{\pi}$ is a fixed point of $\widetilde{T}^{(\lambda)}_\pi$, i.e., $\widetilde{T}^{(\lambda)}_\pi  (V_\pi) = V_\pi.$ 
\end{proposition} 
% \[\rho_{s,a} = \max \{\max_{y\in \widehat{\U}_{s,a}}\min_{x\in \U_{s,a}} \| y-x\|_d, \min_{y\in \widehat{\U}_{s,a}}\max_{x\in \U_{s,a}} \| y-x\|_d \} / d_{\text{min}},~\text{and}~ \rho=\max_{s\in\Ss, a\in\Aa} \rho_{s,a}\]

Intuitively, the convergence of any learning algorithm using the approximate robust TD($\lambda$) operator will depend on the difference between the   actual uncertainty set ${\U}$ and its approximation $\widehat{\U}$. To quantify this, we use the following metric.  Let $\rho=\max_{s\in\Ss, a\in\Aa} \rho_{s,a}$ where 
\begin{align*}
    \rho_{s,a} = \max \hspace{-0.1cm}\left\{\hspace{-0.2cm}\begin{array}{ll} \max_{x\in \widehat{\U}_{s,a}}\max_{y\in {\U}_{s,a} \setminus \widehat{\U}_{s,a}} \| x-y\|_d / d_{\text{min}},\\ \max_{x\in {\U}_{s,a}}\max_{y\in \widehat{\U}_{s,a} \setminus {\U}_{s,a}} \| x-y\|_d / d_{\text{min}} \end{array} \hspace{-0.2cm}\right\} 
\end{align*}
and $d_{\text{min}} := \min_{s \in\Ss} d(s).$ By convention, we set $\rho_{s,a}=0$  when $\widehat{\U}_{s,a} = {\U}_{s,a}$ for all $(s,a)\in(\Ss,\Aa).$ So, $\rho = 0$ if $\widehat{\U} = {\U}$.  Using this characterization and under some additional assumptions on the discount factor, we show that the approximate robust TD($\lambda$) operator  is a contraction in the  $d$-weighted Euclidean norm.
\begin{theorem}
\label{prop:approx-td-op-1}
Under Assumption \ref{as:offpolicy}, for any $V_{1}, V_{2} \in \mathbb{R}^{|\mathcal{S}|}$ and $\lambda \in [0, 1),$ 
\begin{align}
\label{eq:Ttilde-contraction-1} \hspace{-0.3cm}
\|\Pi \widetilde{T}^{(\lambda)}_\pi V_{1} -  \Pi \widetilde{T}^{(\lambda)}_\pi V_{2} \|_{d} \leq  c(\alpha, \beta, \rho, \lambda) ~ \|V_{1} - V_{2}\|_{d}, \hspace{-0.2cm}
\end{align} 
where $c(\alpha, \beta, \rho, \lambda) = {(\beta(2-\lambda) + \rho\alpha  )}/{(1 - \beta  \lambda)}$. So, if $c(\alpha, \beta, \rho, \lambda)  < 1$, $\Pi \widetilde{T}^{(\lambda)}_\pi$ is a contraction in the  $d$-weighted Euclidean norm. Moreover, there exists a unique $w_{\pi}$ such that $\Phi w_{\pi} = \Pi \widetilde{T}^{(\lambda)}_\pi (\Phi w_{\pi})$. Furthermore, for this $w_{\pi}$,
% \begin{align}
% \label{eq:Ttilde-contraction-2}
%     \| V_{\pi} - \Phi  w_{\pi} \|_{d} \leq \frac{1}{\sqrt{1-2(c(\alpha, \beta, \rho, \lambda))^2}} \left(\| V_\pi -  \Pi V_\pi  \|_d  + \sqrt{2}\frac{\beta \rho \| V_\pi\|_d}{1-\beta\lambda} \right)
% \end{align}
\begin{align}
\label{eq:Ttilde-contraction-3}
&\| V_\pi - \Phi w_\pi \|_d \leq \nonumber \\&\hspace{0.2cm}\frac{1}{1 - c(\alpha, \beta, \rho, \lambda)} \left(\| V_\pi -  \Pi V_\pi  \|_d +  \frac{\beta \rho \| V_{\pi}\|_d}{1-\beta\lambda} \right). 
\end{align}
\end{theorem} 
% \redtext{
% \begin{proof}[Proof sketch]
% The key insight which we make towards proving this theorem is to show that the function ${\sigma}_{\widehat{\U}_\pi} (.)$ is $\left(\rho+({\beta}/{\alpha})\right)$-Lipschitz. 
% \end{proof}

% }


%\frac{\beta(2-\lambda) + \rho\alpha  }{(1 - \beta  \lambda)} 
%
%\begin{theorem}
%\label{thm:exist_unique_wopt}
%	Under Assumptions \ref{assum_d} and \ref{assum_op},
%	\begin{align*}
%	\|\Pi{T}^{(\lambda)}_\pi V_{1} -  \Pi{T}^{(\lambda)}_\pi V_{2} \|_{d} \leq \frac{\beta(2-\lambda) + \rho\alpha  }{(1 - \beta  \lambda)} \|V_{1} - V_{2}\|_{d}. 
%	\end{align*} Furthermore, if ${(\beta(2-\lambda) + \rho\alpha  )}/{(1 - \beta  \lambda)}<1$, then there exists a unique $w^{*}$ in $\Phi w^{*} = \Pi {T}^{(\lambda)}_\pi (\Phi w^{*})$.
%\end{theorem}

We note that despite the  assumption on the discount factor, we  empirically show in Section \ref{sec:simulations} that our learning algorithm converges to a robust policy even if this assumption is violated. We also note that the upper bound in \eqref{eq:Ttilde-contraction-3} quantifies the \emph{error} of approximating the robust value function $V_\pi$ with the approximate robust value function $\Phi w_\pi$. We will later use this error bound in in characterizing performance of both RLSPE and RLSPI algorithms. 
% As in \citep{BerBook12,munos2003error,lazaric2012finite}, the \emph{error} bound helps 
% We note that, tightening the contraction mapping  by appropriately modifying the approximate robust TD($\lambda$) operator definition while simultaneously making it amenable to a least squares style online learning algorithm is an interesting  research question. 




Using the contraction property of approximate robust TD($\lambda$) operator, the linear approximation based robust value function $\bar{V}_{\pi} =\Phi w_{\pi}$ can be computed using the iteration, $\Phi w_{k+1} = \Pi \widetilde{T}^{(\lambda)}_{\pi} \Phi w_{k}$. Similar to \eqref{eq:rpvi-11},  we can get a closed form solution for $w_{k+1}$  using \textbf{least squares approach}  as
\begin{align}
\label{eq:rpvi-approx-1}
\hspace{-0.2cm} w_{k+1} = w_{k} + (\Phi^{\top} D \Phi)^{-1} \Phi^{\top} D (\widetilde{T}^{(\lambda)}_{\pi} \Phi w_{k}  - \Phi w_{k}).
\end{align}
This can be written in a more succinct matrix form as given below (derivation is given in the supplementary material).
\begin{align}
\label{eq:rpvi-approx-matrix-1}
w_{k+1} &= w_{k} + B^{-1}(A w_{k} +  C(w_{k}) + b),~~ \text{where}, \\
\label{eq:AB-1}
&A =  \Phi^{\top} D  (\alpha P^{o}_{\pi} - I) \sum^{\infty}_{m=0}  (\alpha \lambda P^{o}_{\pi})^{m}  \Phi,  \\
&B =   \Phi^{\top} D \Phi, \\ \label{eq:Cb-1}
&C(w) = \alpha \Phi^{\top} D  \sum^{\infty}_{t=0} (\alpha \lambda P^{o}_{\pi})^{t}  {\sigma}_{\widehat{\U}_{\pi}} (\Phi w), \\ &  b = \Phi^{\top} D  \sum^{\infty}_{t=0} (\alpha \lambda P^{o}_{\pi})^{t} r_{\pi}.
\end{align}
Iterations by evaluating \eqref{eq:rpvi-approx-matrix-1} exactly is intractable for MDPs with large state space, and infeasible if we do not know the transition probability $P^{o}_\pi$. To address this issue, we propose a simulation-based model-free online reinforcement learning algorithm, which we call robust least squares policy evaluation (RLSPE($\lambda$)) algorithm, for learning the robust value function. 

{\bf RLSPE($\lambda$) algorithm:} Generate a sequence of states and rewards, $(s_{t}, r_{t}, t \geq 0),$ using  the policy $\pi$. Update the parameters as
\begin{align}
\label{eq:RLSPE-1}
&\hspace{-0.2cm}w_{t+1} = w_{t} + \gamma_{t} B^{-1}_{t}(A_{t} w_{t} + b_{t} + C_{t}(w_{t})),~ \text{where},\\
% \end{align}
% 	\begin{align}
\label{eq:AB-2}
&A_t = \frac{1}{t+1} \sum_{\tau=0}^{t} z_{\tau} ~ (\alpha \phi^{\top}(s_{\tau + 1}) - \phi{^\top}(s_\tau)), \\ &B_t = \frac{1}{t+1} \sum_{\tau=0}^{t} \phi(s_\tau) \phi{^\top}(s_\tau),\\
&C_t(w) = \frac{\alpha}{t+1}  \sum_{\tau=0}^{t} z_{\tau}  ~ \sigma_{\widehat{\U}_{s_{\tau}, \pi(s_{\tau})}} ( \Phi w), \\&b_t = \frac{1}{t+1}  \sum_{\tau=0}^{t}  z_{\tau}  r(s_{\tau},\pi(s_{\tau})),\\ &z_{\tau} = \sum_{m=0}^{\tau} (\alpha \lambda)^{\tau-m} \phi(s_{m}), \label{eq:z-2}
\end{align}
where $\gamma_{t}$ is a deterministic sequence of step sizes. We assume that the step size satisfies the  the standard Robbins-Munro stochastic conditions for stochastic approximation, i.e., $\sum^{\infty}_{t=0} \gamma_{t} = \infty,~ \sum^{\infty}_{t=0} \gamma^{2}_{t} < \infty$. 

We use the on-policy version of the RLSPE($\lambda$) algorithm in the above description. So,  we implicitly assume that the given policy $\pi$ is an exploration policy according to the Assumption \ref{as:offpolicy}. This is mainly for the clarity of the presentation and notational convenience. Also, this simplifies the presentation of the policy iteration algorithm introduced in the next section.  An  off-policy version of the above algorithm can be implemented using the techniques given in \citep{bertsekas2009projected}. We now give the convergence result of the RLSPE($\lambda$) algorithm. 
\begin{theorem}
\label{thm:RLSPE-convergence-1}
Let Assumption \ref{as:offpolicy} hold. Also, let $c(\alpha, \beta, \rho, \lambda) < 1 $ so that $\Pi \widetilde{T}^{(\lambda)}_{\pi}$ is a contraction according to Theorem \ref{prop:approx-td-op-1}.  Let $\{w_{t}\}$ be the sequence generated by the RLSPE($\lambda$) algorithm given in \eqref{eq:RLSPE-1}. Then,  $w_{t}$ converges to $w_{\pi}$  with probability 1 where $w_{\pi}$ satisfies the fixed point equation $\Phi w_{\pi}= \Pi \widetilde{T}^{(\lambda)}_{\pi} \Phi w_{\pi}$.
\end{theorem}

The key idea of the proof is to show that the RLSPE($\lambda$) update \eqref{eq:RLSPE-1} approximates the exact update equation \eqref{eq:rpvi-approx-1} and both converge to the same value $w_{\pi}$. One particularly challenging task is in analyzing the behavior of the term $C_{t}(w)$ due to the non-linearity of the function ${\sigma}_{\widehat{\U}_\pi} (.)$. We use the tools from stochastic approximation theory \citep{borkar2009stochastic, nedic2003least} to show this rigorously after establishing the tractable properties of the function ${\sigma}_{\widehat{\U}_\pi} (.)$. 

Note that Theorem \ref{thm:RLSPE-convergence-1} and  Theorem \ref{prop:approx-td-op-1} together give an error bound for the converged solution of the RLSPE($\lambda$) algorithm. More precisely,  Theorem \ref{thm:RLSPE-convergence-1} shows the convergence of the  RLSPE($\lambda$) algorithm to $w_{\pi}$ and Theorem \ref{prop:approx-td-op-1} gives the bound on $\| V_\pi - \Phi w_\pi \|_d$, which is the error due to linear function approximation. We will use this bound in the the convergence analysis of  the RLSPI algoirthm presented in the next section.

% \redtext{ \begin{proof}[Proof sketch]
% The proof of this theorem relies on verifying the sufficient conditions in the stochastic approximation result \citep[Proposition 4.1]{nedic2003least}. Our proposed approximate robust TD($\lambda$) operator in \eqref{eq:TLambda-1} as opposed to the robust TD($\lambda$) operator in \eqref{eq:TLambda-Ber-1} becomes crucial in proving this theorem. In particular, the function ${\sigma}_{\widehat{\U}_\pi} (.)$ being $\left(\rho+({\beta}/{\alpha})\right)$-Lipschitz helps in this first-order proof methodology employed in the stochastic approximation update equations. 
% \end{proof} }


==> ICML 2021 Submission/04-LSPI.tex <==
\section{Robust Least Squares Policy Iteration}
\label{sec:PI}

In this section, we introduce the robust least squares policy iteration (RLSPI) algorithm for finding the optimal robust policy.  RLSPI algorithm can be thought as the robust version of the  LSPI algorithm \citep{lagoudakis2003least}. RLSPI algorithm uses the RLSPE($\lambda$) algorithm for policy evaluation. However, model-free policy improvement is difficult when working with value functions since the policy update step will require us to solve \begin{align}
\label{eq:policy_update_value}
\pi_{k+1}  =  \argmax_{\pi}\widetilde{T}^{(\lambda)}_{\pi} (\bar{V}_k),
\end{align} where $\bar{V}_k$ is the approximate robust value function corresponding to the policy $\pi_k$, in the $(k+1)^{\text{th}}$ policy iteration loop. To overcome this, we first introduce the robust state-action value function (Q-function). 

For any given policy $\pi$ and  state-action pair $(s,a)$, we define the robust $Q$-value as,
\begin{align}
    \hspace{-0.3cm}Q_{\pi}(s,a) = \inf_{P \in \mathcal{P}}  \mathbb{E}_{P}[\sum^{\infty}_{t=0} \alpha^{t} r(s_{t}, a_{t}) ~| s_{0} = s, a_{0} =a].\hspace{-0.2cm}
\end{align}
Instead of learning the approximate robust value function $\bar{V}_{\pi}$, we can learn the approximate robust Q-value function $\bar{Q}_{\pi}$  using RLSPE($\lambda$). This can be done by defining the feature vector $\phi(s,a)$ where  $\phi(s,a) = (\phi_{1}(s,a), \ldots, \phi_{L}(s,a))^{\top}$ and the linear approximation of the form $\bar{Q}_{\pi}(s, a) = w^{\top} \phi(s,a)$ where  $w$ is a weight vector. The results from the previous section on the convergence of the RLSPE($\lambda$) algorithm applies for the case of learning Q-value function as well. 

RLSPI is a policy iteration algorithm that uses RLSPE($\lambda$) for policy evaluation at each iteration. It starts with an arbitrary initial policy $\pi_{0}$. At the $k$th iteration, RLSPE($\lambda$) returns a weight vector that represents the approximate Q-value function $\bar{Q}_{\pi_{k}} = \Phi w_{\pi_{k}} $ corresponding to the policy $\pi_{k}$. The next policy $\pi_{k+1}$ is the greedy policy corresponding to $\bar{Q}_{\pi_{k}}$, defined as $\pi_{k+1}(s) = \argmax_{a \in \mathcal{A}} \bar{Q}_{\pi_{k}}(s,a)$. For empirical evaluation purposes, we terminate the policy iteration for some finite value $K.$ RLSPI algorithm is summarized in Algorithm \ref{algo-lspI}.

\begin{algorithm}
	\caption{RLSPI Algorithm} 
	\label{algo-lspI}
	\begin{algorithmic}[1]
		\STATE Initialization: Policy evaluation weights error $\epsilon_0$, initial policy $\pi_0$. 
		\FOR {$k=0 \ldots K$}
		\STATE Initialize the policy weight vector $w_{0}$. Initialize time step $t \leftarrow 0.$
		    \REPEAT
		        \STATE Observe the state $s_{t},$ take action $a_{t} = \pi_{k}(s_{t}),$ observe  reward $r_{t}$ and  next state $s_{t+1}$.
		        \STATE Update the weight vector $w_{t}$ according to RLSPE($\lambda$) algorithm  (c.f. \eqref{eq:RLSPE-1}-\eqref{eq:z-2})
		        \STATE $t \leftarrow t+1$
		    \UNTIL{$\|w_{t}-w_{t-1}\|_2 < \epsilon_0$}
		    \STATE $w_{\pi_{k}} \leftarrow w_{t}$
		    \STATE Update the policy $$\pi_{k+1}(s) = \argmax_{a \in \mathcal{A}} \phi(s,a)^{\top} w_{\pi_{k}}$$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}


We make the following assumptions for the convergence analysis of the RLSPI algoirthm. We note that we work with value functions instead of Q-value functions for notational convenience and consistency. 


\begin{assumption}
\label{as:policy_iteration_req} (i) Each policy $\pi_{k}$ is an exploration policy, i.e. $\pi_{\text{exp}}(\pi_{k}) = \pi_{k}$.\\
(ii) The Markov chain $P^{o}_{\pi_{k}}$ has a stationary distribution $d_{\pi_{k}}$ such that $d_{\pi_{k}}(s) > 0, \forall s \in \mathcal{S}.$ \\
(iii) There exists a finite scalar $\delta$ such that ~$ \|V_{\pi_{k}} - \Pi_{d_{\pi_{k}}} V_{\pi_{k}} \|_{d_{\pi_{k}}}  < \delta$ for all $k$, where $\Pi_{d_{\pi_{k}}}$ is a projection onto the subspace spanned by the columns of $\Phi$ under the $d_{\pi_{k}}$-weighted  Euclidean norm. \\ % $\max \{ \|V_{\pi_{k}} \|_{d_{\pi_{k}}},\|V_{\pi_{k}} - \Pi_{d_{\pi_{k}}} V_{\pi_{k}} \|_{d_{\pi_{k}}} \} < \delta$ for all $k$.
(iv) For any probability distribution $\mu$, define probability another distribution $\mu_k = \mu H_k $ where $H_k$ is a stochastic matrix defined with respect to $\pi_{k}$. Also assume that there exists a probability distribution $\bar{\mu}$ and finite positive scalars $C_{1}, C_{2}$ such that $\mu_{k} \leq C_{1} \bar{\mu}$ and $d_{\pi_{k}} \geq \bar{\mu}/C_{2}$ for all $k$. 
\end{assumption}







We  note that these are  the standard assumptions used in the RL literature to provide theoretical guarantees for approximate policy/value iteration algorithms with linear function approximation in the non-robust settings \citep{munos2003error,munos08a, lazaric2012finite}.  We make no additional assumptions even though we are addressing the  more difficult robust RL problem. The specific form of the stochastic matrix $H_k$ specified in Assumption \ref{as:policy_iteration_req}.$(iv)$ is deferred to the proof of Theorem \ref{thm:RLSPI} for brevity of the presentation. 



We now give the asymptotic convergence result for the RLSPI algorithm. We assume that, similar to the non-robust setting \citep{munos2003error}, the policy evaluation step (inner loop) is run to the convergence. 
We only present the case where $\rho = 0$. The proof for the general case is straightforward, but involves much more detailed algebra. So, we omit those details for the clarity of presentation. 
\begin{theorem}
\label{thm:RLSPI}
Let Assumption \ref{as:offpolicy} and Assumption \ref{as:policy_iteration_req} hold. Let $\{\pi_{k}\}$  be the sequence of the policies generated by the RLSPI algorithm. Let $V_{\pi_{k}}$ and $\bar{V}_{k} = \Phi w_{\pi_{k}}$ be true robust value function and the approximate robust value function corresponding to the policy $\pi_{k}$. Also, let  $V^*$ be the optimal robust value function. Then, with $c(\alpha,\beta,0,\lambda)<1$,
\begin{align} \label{eq:pi_thm_1}
    &\hspace{-0.2cm}\limsup_{k\to\infty} \| V^* - V_{\pi_k} \|_\mu\nonumber\\&\hspace{-0.1cm}\leq \frac{2\sqrt{C_1 C_2}~c(\alpha,\beta,0,\lambda) }{(1-c(\alpha,\beta,0,\lambda) )^2}~ \limsup_{k\to\infty} \|V_{\pi_{k}} - \bar{V}_{k}\|_{d_{\pi_k}}.
\end{align}
Moreover, from Theorem \ref{prop:approx-td-op-1} and  Assumption \ref{as:policy_iteration_req}.$(iii)$,   we have
\begin{align} \label{eq:pi_thm_2}
    \limsup_{k\to\infty} \| V^* - V_{\pi_k} \|_\mu\leq  \frac{2\sqrt{C_1 C_2}~c(\alpha,\beta,0,\lambda) }{(1-c(\alpha,\beta,0,\lambda) )^3}~ \delta  .
\end{align}
\end{theorem}

The above theorem, in particular \eqref{eq:pi_thm_2}, gives a (worst case) guarantee for the performance of the policy learned using the RLSPI algorithm. Note that the upper bound in \eqref{eq:pi_thm_2} is a constant where $\delta$ represents the (unavoidable) error due to the linear function approximation. We also note that using `$\limsup$' is necessary due to the policy chattering phenomenon in approximate policy iteration algorithms which exists even in the non-robust case \citep{BerBook12}. 

Instead of the asymptotic bound given in Theorem \ref{thm:RLSPI}, we can actually get a bound for any $K$ given in the RLSPI algorithm by modifying Assumption \ref{as:policy_iteration_req}.$(iv)$. We defer the precise statements of the assumption and theorem to  Section \ref{sec:PI_appendix} in the supplementary material due to page limitation.


 


% \begin{assumption}\label{as:finite_time_pi}
% For an arbitrary sequence of stationary policies $\{\pi_i\}_{i\geq 1}$, let some probability distributions $\mu$ and $\bar{\mu}$ satisfy
% \begin{align}
%     \frac{C_{\mu,\bar{\mu}}}{(1-c(\alpha,\beta,0,\lambda))} =  \sum_{m\geq 1} (c(\alpha,\beta,0,\lambda))^m c_{\mu,\bar{\mu}}(m) < \infty, \label{eq:C_mu}
% \end{align} where for any given $m\geq 1$ the coefficients are defined as \begin{align}
%     c_{\mu,\bar{\mu}}(m) = \sup_{\pi_1,\ldots,\pi_m} \left\| \frac{\dd(\mu \bar{H}_1\bar{H}_2\ldots\bar{H}_m)}{\dd\bar{\mu}} \right\|_\infty, \label{eq:c_mu_coefficients}
% \end{align}
% and $\bar{H}_k$ is a stochastic matrix that depends on $P^o_{\pi_{k}}$ for any $1\leq k \leq m$. Also assume that $d_{\pi_{k}} \geq \bar{\mu}/C$ for all $k$. 
% \end{assumption}

% We note that $c_{\mu,\bar{\mu}}(m)$ can potentially diverge to $\infty$, but $C_{\mu,\bar{\mu}}$ is finite as long as $(c(\alpha,\beta,0,\lambda))^m$ converges to $0$ at a faster rate. Assumption \ref{as:finite_time_pi} being similar as in the non-robust setting, for a detailed interpretation of it, we refer the reader to \citep{antos2008learning,lazaric2012finite}. %The specific form of the stochastic matrix $\bar{H}_k$ specified in Assumption \ref{as:policy_iteration_req}.$(iv)$ is deferred to the proof of Theorem \ref{thm:RLSPI} for the brevity of the presentation. 

% \begin{theorem}[informal]
% \label{thm:RLSPI_for_any_K}
% Let Assumption \ref{as:offpolicy}, Assumption \ref{as:policy_iteration_req}.(i)-(iii), and Assumption \ref{as:finite_time_pi} hold. Let the range of reward function $r$ be $(0,R_{\max}]$. Let $\{\pi_{k}\}_{k=1}^K$  be the sequence of policies generated by the RLSPI algorithm for some $K\geq 1$. %Let $V_{\pi_{k}}$ and $\bar{V}_{k} = \Phi w_{\pi_{k}}$ be true robust value function and the approximate robust value function corresponding to the policy $\pi_{k}$. Also, let  $V^*$ be the optimal robust value function. 
% Then, with $c(\alpha,\beta,0,\lambda)<1$,
% \begin{align*} 
%     &\hspace{-0.2cm} \| V^* - V_{\pi_K} \|_\mu\nonumber\leq \frac{2\sqrt{2} (c(\alpha,\beta,0,\lambda))^{(K+1)/2} }{(1-c(\alpha,\beta,0,\lambda) )^{3/2}}~ R_{\max}  \\&\hspace{-0.1cm}+ \frac{2\sqrt{2} c(\alpha,\beta,0,\lambda) \sqrt{C C_{\mu,\bar{\mu}}} }{(1-c(\alpha,\beta,0,\lambda) )^2} \max_{0\leq k < K} \|V_{\pi_{k}} - \bar{V}_{k}\|_{d_{\pi_k}}.
% \end{align*}
% % Moreover, from Theorem \ref{prop:approx-td-op-1} and  Assumption \ref{as:policy_iteration_req}.$(iii)$, as $K\to\infty$  we have
% % \begin{align} 
% %     \| V^* - V_{\pi_K} \|_\mu\leq  \frac{2\sqrt{2} c(\alpha,\beta,0,\lambda) \sqrt{C C_{\mu,\bar{\mu}}} }{(1-c(\alpha,\beta,0,\lambda) )^3} ~ \delta  .
% % \end{align}
% \end{theorem}

==> ICML 2021 Submission/05-Simulations.tex <==
\section{Experiments} \label{sec:simulations}

\begin{figure*}[t]
% \vspace{-0.2cm}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{randomaction_cart.pdf}
		\captionof{figure}{CartPole}
		\label{fig:cart_failprob}
	\end{minipage}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{randomaction_mt_.pdf}
		\captionof{figure}{MoutainCar}
		\label{fig:mt_failureprob}
	\end{minipage}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{acro_failureprob.pdf}
		\captionof{figure}{Acrobot}
		\label{fig:acro_failureprob}
	\end{minipage}
% \end{figure*}
% \begin{figure*}[t]
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{force_cart.pdf}
		\captionof{figure}{CartPole}
		\label{fig:cart_force-in}
	\end{minipage}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{gravity_cart.pdf}
		\captionof{figure}{CartPole}
		\label{fig:cart_gravity-in}
	\end{minipage}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{polelength_cart.pdf}
		\captionof{figure}{CartPole}
		\label{fig:cart_pole-in}
	\end{minipage}
\end{figure*}

We implemented our RLSPI algorithm using the MushroomRL library \citep{deramo2020mushroomrl}, and evaluated its performance against  Q-learning algorithm for an environment with discrete action space, deep deterministic policy gradient (DDPG) \citep{lillicrapHPHETS15} algorithm for continuous action space, and LSPI algorithm  \citep{lagoudakis2003least}.  For comparing with the performance of our RLSPI algorithm against another robust RL algorithm, we implemented the  soft-robust algorithms proposed in \citep{derman2018soft} which use deep neural networks for function approximation. 


We chose a spherical uncertainty set with a radius $r$. For such a set $\widehat{\mathcal{U}}$, a closed form solution of $\sigma_{\widehat{\mathcal{U}}}(\Phi w)$ can be computed for faster simulation.  We note that in all the figures shown below, the quantity in the vertical axis is averaged over $100$ runs, with the thick line showing the averaged value and the band around shows the $\pm 0.5$ standard deviation. These figures act as the performance criteria for comparing results. We provide more details and additional experiment results in Section \ref{sec:experiments} of supplementary. 

We used the CartPole, MountainCar, and Acrobot environments from  OpenAI Gym \citep{brockman2016openai}. We trained LSPI algorithm and our RLSPI algorithm on these environments with nominal parameters (default parameters in OpenAI Gym \citep{brockman2016openai}). We also trained Q-learning with linear function approximation and soft-robust deep Q-network(DQN) \citep{derman2018soft} algorithms on CartPole environment, DQN and soft-robust DQN \citep{derman2018soft} algorithms on Acrobot environment, and DDPG and soft-robust DDPG \citep{derman2018soft} algorithms on MountainCar environment. Then, to evaluate  the robustness of the polices obtained, we changed the parameters of these environments and tested the performance of the learned polices on the perturbed environment. 

In Figures \ref{fig:cart_failprob}-\ref{fig:acro_failureprob}, we show the robustness against  action perturbations. In real-world settings, due to model mismatch or noise in the environments, the resulting action  can be different from the intended action. We model this by picking a random action with some probability at each time step. Figure \ref{fig:cart_failprob} shows the  change in  the average episodic reward against the probability of picking a random action for the CartPole environment.  Figure \ref{fig:mt_failureprob} shows the average number of time steps to reach the goal in the MountainCar environment. Figure \ref{fig:acro_failureprob} shows the average episodic reward in the Acrobot environment. In all three cases,  RLSPI algorithm shows robust performance against the perturbations.  


Figures \ref{fig:cart_force-in}-\ref{fig:cart_pole-in} shows the test performance on CartPole, by changing the parameters  \emph{force$\_$mag} (external force disturbance), \emph{gravity}, \emph{length} (length of pole on the cart). The nominal values of these parameters  are $10, 9.8$, and  $0.5$ respectively. RLSPI again exhibits robust performance.  

The performance of our RLSPI algorithm is consistently superior to that of the non-robust algorithms. Moreover, the performance of RLSPI algorithm is  comparable  with that of the soft-robust algorithms \citep{derman2018soft}, even though the latter uses deep neural networks for function approximation while our algorithm uses only linear function approximation architecture. We also would like to emphasize that our work gives provable guarantees for the policy learned by  the algorithm whereas \citep{derman2018soft} does not provide any such guarantees.  





==> ICML 2021 Submission/06-Conclusions.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
We have presented an online model-free reinforcement learning algorithm to learn control policies that are robust to the parameter uncertainties of the model, for system with large state spaces. While there have been  interesting empirical works on robust deep RL using neural network, they only provide  convergence guarantees to a local optimum. Different from such empirical works, we proposed a learning based robust policy iteration algorithm called RLSPI algorithm with explicit theoretical guarantees on the performance of the learned policy. To the best of our knowledge, this is the first work that presents  model-free reinforcement learning algorithm  with function approximation for learning the optimal robust policy.  We also empirically evaluated the performance of our RLSPI algorithm on standard benchmark RL problems. 



In  future, we plan to extend our theoretical results to nonlinear function approximation architectures. We also plan to characterize the  sample complexity of robust reinforcement learning algorithms. Extending offline RL approaches to robust setting is another research area that we plan to pursue. 


% more viable structures for tractable RMDP formulations. We also plan to address this problem  using offline reinforcement learning techniques, for improving the data efficiency. Off-policy policy gradient methods for robust reinforcement is another exciting but challenging direction.


%  for the uncertainty sets leading to other interesting approximate robust TD($\lambda$) operators


